FluxShard: Motion-Aware Feature Cache Reuse for Collaborative Video Analytics in Mobile Edge Computing

Caching and reusing intermediate features across consecutive frames is a common technique to reduce redundant computation and transmission for edge-cloud video analytics in mobile edge computation. Existing methods manage the cache in a fixed or globally shifted coordinate system, treating it as an indivisible whole. Under the non-uniform motion patterns of mobile scenes, this whole-scene granularity invalidates large portions of the cache even when most content has merely shifted spatially, wasting computation and bandwidth. The root cause is a granularity mismatch: the cache is managed per scene, yet motion varies per region. In this paper, we present FluxShard, a motion-aware edge-cloud video analytics system that uses codec-level block motion vectors (MVs) to manage feature cache reuse and recomputation at the granularity of individual motion regions. By re-indexing cached features along per-block MVs, FluxShard separates spatial displacement from content changes, recovering reusable content that whole-scene methods would otherwise discard. To ensure correct reuse under heterogeneous motion, the Receptive Field Alignment Principle (RFAP) identifies, from the input-level MV field alone, the positions that must be recomputed due to inconsistent spatial composition within receptive fields. To maintain cache coherence across frames, MV-guided cache remapping warps the entire feature cache to the current coordinate system each frame, sustaining a high reuse ratio over time. A profiling-driven dispatcher routes the remaining sparse workload between edge and cloud for lower latency. Evaluation across multiple vision tasks, dynamic video benchmarks, and network conditions shows that FluxShard reduces latency by 32.6-83.8% and energy by 14.9-64.0% over all baselines under the prescribed accuracy budget.

==> src/impl.tex <==
\section{Implementation}\label{sec:impl}

We prototype FluxShard on an NVIDIA Jetson Xavier NX (edge) and an NVIDIA RTX 3080 GPU (cloud), connected over a TCP link whose bandwidth is shaped with \texttt{tc} to emulate cellular uplink conditions.

\paragraph{State management and offload reconstruction}
The client maintains two dispatch-layer states as described in \S\ref{sec:pipeline}.
When a frame is offloaded, the client sends the cloud state's accumulated MV field, a packed recomputation mask, and the recomputation RGB pixels.
The server reconstructs the sparse input from these payloads and its cached reference, applies the RFAP check, runs sparse inference, and performs cache remapping.
After transmission, the client mirrors the same cloud-state update to keep both sides synchronized.

\paragraph{RFAP consistency check}
A custom CUDA kernel implements the RFAP check (Conditions~1 and~2 in \S\ref{sec:rfap}) directly from the accumulated MV field, producing a binary mask merged into the recomputation set at the first spatial layer.

\paragraph{Sparse inference engine}
We store all feature tensors in channel-last (NHWC) layout throughout the sparse path, matching FluxShard's per-position access pattern and avoiding layout conversion overhead.

We implement sparse convolution, pooling, and activation with custom CUDA kernels.
The convolution kernel follows an implicit-GEMM structure with the same dense-style load and store pattern as the dense counterpart, but skips arithmetic at inactive positions.
At activation layers, truncation, MV-guided history lookup, and history refresh are fused into a single pass, so cache maintenance does not require a separate remapping kernel.
On fully dense inputs, the custom convolution kernel approaches cuDNN-level throughput; as sparsity increases, execution time decreases nearly proportionally.

\paragraph{Offload metadata}
FluxShard uses $16\times16$ MV blocks, so with two 16-bit components (int16) per block, the MV field occupies approximately 0.52\% of the full RGB input in 8-bit format (uint8).
For offloading, we further downsample the recomputation mask by $2\times2$ and pack it bitwise before transmission.
The packed mask occupies approximately 1.04\% of the input.
Together, the MV field and mask contribute only 1.56\% metadata overhead before the recomputation RGB pixels themselves are transmitted.
These ratios are independent of the absolute input resolution.


==> tmp/generated/e2e_workload_reference.tex <==
Dense local execution on the Jetson Xavier NX takes 557.4$\pm$38.5\,ms and 8.11$\pm$0.94\,J per segmentation frame, and 445.5$\pm$10.5\,ms and 6.81$\pm$0.19\,J per pose frame. In contrast, dense cloud inference alone takes 35.7$\pm$3.0\,ms for segmentation and 27.6$\pm$3.0\,ms for pose on the RTX 3080; the end-to-end penalty of pure offload is therefore dominated by network transport rather than server compute.

